Intrinsic structure of liquid surface and capillary waves on the Density Functional Theory

Two different theories are used to understand the liquid-vapor interfaces: the Van der Waals theory and the capillary waves theory. But comparing both come up a problem of interpretation of the interface density profiles obtained, for example, with the Density Functional Theory (DFT). As a consequence emerge the question of how the surface fluctuations are included on traditional density profiles (usually named equilibrium density profiles). Last years, new insights on the role of capillary waves were possible by analyzing X-ray reflectivity experiments and performing computer simulations of liquids with low melting temperature. In particular, the density profile exhibits a layering structure which is considered a key property to elucidate a new interpretation of those profiles as intrinsic density profiles. This dissertation aims to investigate these questions within the DFT using simple fluids with a pairwise interactions that reproduce important phase-diagram properties of liquid metals. Two generics questions were explored: the relevance of Fisher-Widom line and the role of capillary waves on the nature of interface obtained with approximations WDA and FMT. It hypothesized the existence of a density profile with strong layering properties whose structure is reduced by capillary waves. Then the effect of surface fluctuations is described by introducing an effective transversal size which imposes a limitation of the spectrum of surface fluctuations incorporated on the DFT. However, an explicit methodology to unfreeze the capillary waves over a postulated intrinsic profile exempt of surface fluctuations was proven still a challenge. As a consequence it suggested that other previous results describing the liquid surface using the equilibrium DFT may conduct to unphysical properties.

==> 32Perfilesdensidad.tex <==
\section{Determinación del perfil de densidad líquido-vapor}
Todo el conjunto de formalismo desarrollados hasta el momento permiten en teoría la determinación por diferentes métodos del perfil de densidad en una interfase. Del conjunto de relaciones la primera vía usada para la determinación del perfil de densidad fue resolver la ecuación de YBG que expresa el perfil de densidad como una ecuación iontegral autoconsistente donde la principal dificultad es la determinación de $g^{2}$, que es la función que contiene toda la información de la transición de fase. El desconocimiento de esta función hace analizar el problema basandose en el conocimiento del caso homogeneoy y basando en la aproximación que vimos $g(r_{12};\bar{rho})$, donde para un potencial generico tampoco se conoce pero hemos visto que estructuralmente el desarrollo entorno del potencial de esferas duras es muy eficaz. Es interesante recuperar las diferentes propuestas para $\bar{\rho}$ y las propuestas para el shift en z que se produce en el perfil, usualmente se procedia recalculando la superficie de Gibbs en cada paso, pero tal y como apuntaba Croxton esto puede llevar a eliminar la presencia real de oscilaciones en el perfil de densidad del fluido, que como veremos es una caracteristica esencial del problema de las interfase liquidas.\\

Igualmente se puede hacer una aproximación integral basada en la función de correlación directa que como veremos es más natural para obtener estructuras oscilantes. Pero la solución directa para los perfiles de densidad se ha obtenido de teorias generalizadas de van der Waals en el contexto del funcional de la densidad.\\

Es resaltable el trabajo realizado por Croxton, en la ecuación de BBYG que posee una la filosifía similar a esta ecuación. Su objetivo fue encontrar expresiones plausibles para las funciones de distribución en la interfase, proponiendo de hecho, una densidad oscilante en la parte densa del perfil de densidad\cite{0022-3719-4-14-005}\cite{0022-3719-4-16-009}\cite{0022-3719-4-14-006} y constituye por tanto la primera aportación en el contexto de la teoría de liquidos desde el enfoque que al problema de la interfase se dan en esta memoria. Croxton observa como bajo BBYG, como aqui, tenemos que incluir el conocimiento de la funcion de distribución a dos cuerpos, dificil de conocer en el caso no-homogeneo y propone incluir un operador que transforme el caso homogeneo en el caso no-homogeneo y resolver así una expresion para la función de distribución a un cuerpo bajo hipotesis plausubles para este operador. En su trabajo de hecho intuye que en los metales liquidos la estructuración deberia ser más equivente que en el caso del Argón estudiado por él. Más adelante se han determinado también bajo la ecuación BGYB estructuras liquidas en contacto con paredes\cite{PhysRevA.22.2836}, sin embargo hasta el desarrollo de funcionales de la densidad que incluian mejores aproximaciones a las correlaciones del sistema de esferas duras no se vislubra la evidencia de perfiles estructurados y se retoma la imagen dada por Croxton\cite{EvansMolecularPhyscFWline}.

